Semi-Supervised Multimodal Multi-Instance Learning for Aortic Stenosis Diagnosis

Automated interpretation of ultrasound imaging of the heart (echocardiograms) could improve the detection and treatment of aortic stenosis (AS), a deadly heart disease. However, existing deep learning pipelines for assessing AS from echocardiograms have two key limitations. First, most methods rely on limited 2D cineloops, thereby ignoring widely available Doppler imaging that contains important complementary information about pressure gradients and blood flow abnormalities associated with AS. Second, obtaining labeled data is difficult. There are often far more unlabeled echocardiogram recordings available, but these remain underutilized by existing methods. To overcome these limitations, we introduce Semi-supervised Multimodal Multiple-Instance Learning (SMMIL), a new deep learning framework for automatic interpretation for structural heart diseases like AS. When deployed, SMMIL can combine information from two input modalities, spectral Dopplers and 2D cineloops, to produce a study-level AS diagnosis. During training, SMMIL can combine a smaller labeled set and an abundant unlabeled set of both modalities to improve its classifier. Experiments demonstrate that SMMIL outperforms recent alternatives at 3-level AS severity classification as well as several clinically relevant AS detection tasks.

==> Ablation_FullSet.tex <==
\begin{table}[h]
    \caption{Ablation. AS Severity Classification on TMED2 (Full-set). Showing balanced accuracy on the test set across three predefined train/test splits.
    }%endcaption
    \centering % Add this to center the table
    \begin{tabular}{l|rrr| r }
	    & \multicolumn{4}{c}{Test Set Bal. Accuracy}\\
     Method & split 1 & split 2 & split 3 & average (std)\\
    \hline
    SMMIL (video-based) & \textbf{83.13} & \textbf{80.62} & \textbf{86.59} & \textbf{83.45} (2.45)\\
    SMMIL (video-based) (no SSL) & 79.77 & 77.72 & 81.65 & 79.71 (1.60)\\
    SMMIL (video-based) (no doppler) & 72.97 & 75.28 & 73.74 & 74.00 (0.96)\\
    \end{tabular}
    \\
    \label{tab:TMED2_BACC_FullSet_Ablation}
\end{table}

==> CleanSet_ClassificationResults.tex <==
\begin{table}[h]
    \caption{AS Severity Classification on TMED2 (clean-set). Showing balanced
    accuracy on the test set across three predefined train/test splits. ``--'' means not reported in the cited papers. \textbf{For the medical foundation models, we evaluate on an easier No vs Some AS binary classification task, where chance performance is 50\%}
    }%endcaption
    \centering % Add this to center the table
    \begin{tabular}{l|rrr| r }
	    & \multicolumn{4}{c}{Test Set Bal. Accuracy}\\
     Method & split 1 & split 2 & split 3 & average (std)\\
    \hline
    W. Avg~\cite{wessler2023automated} 
    & 74.46 & 72.61 & 76.24 & 74.43 (1.48) \\
    ProtoASNet~\cite{vaseli2023protoasnet} 
    & 79.70 & --& -- & -- \\
    Transformer-based Echo~\cite{ahmadi2023transformer} 
    & 83.80 & -- & -- & -- \\
    \hline
    Med-Flamingo (zero-shot) 
    & 50.00 & 50.00 & 50.00 & 50.00 (0) \\
    Med-Flamingo (COT) 
    & 50.00 & 50.00 & 50.00 & 50.00 (0) \\
    RadFM (zero-shot) 
    & 60.36 & 53.30 & 56.01 & 56.56 (2.91) \\
    \hline
    SMMIL (ours, image-based) & \emph{86.65} & \emph{82.78} & \textbf{87.66} & \emph{85.70} (2.10)\\
    SMMIL (ours, video-based) & \textbf{87.69} & \emph{82.14} & \textbf{89.63} & \textbf{86.49} (3.17)\\
    \end{tabular}
    \\
    \label{tab:TMED2_BACC_Cleanset}
\end{table}

==> LLM_Scratch.tex <==
\subsection{Evaluation of Large Language Model has taken thw world by storm. Foundation Model with Prompting}
The term “foundational models” was first introduced by Bommasani et al.~\cite{bommasani2021opportunities} defined as “the
base models trained on large-scale data in a self-supervised or
semi-supervised manner that can be adapted for several other
downstream tasks”. with the goal to perform well both in-domain and out-domain.
(e.g., CLIP show good zero-shot generalization, RadFM tested its ability on zero-shot generalization on disease class not trained on)

Common ways to utilize foundation models include Supervised Finetuning (SFT), Retrival Augmented Generation (RAG), a technique for enhancing the accuracy and reliability of generative AI with facts fetch from external source, and Prompting Engineering, where prompt engineering is usually the first thing to try, as it is most accessible, while the other two techniques has substaintially higher barrier such as substaintial computation cost and complicated procedures ~\cite{gruver2023large}.

Large Language Model (LLM) such as ChatGPT has taken the world by storm. With the rise of LLM, 
the development of large models (e.g., language/vision/language-vision multi-modal) has gathered unparallel interest in the machine learning community. Recently, such efforts have been expanded to the medical domain~\cite{moor2023med,wu2023towards,liu2023qilin}, with the goal to develop foundation/generalist model that can perform well on various medical task at the same time and even generalize to unseen task. In the language of LLM era, most of the existing models, including this paper, are called ``specialist model'', as they specialize only a handful of tasks at a time. 


Moreover, recent study has highlight that in some cases, prompting can achieve comparable performance to the more costly SFT. 

The goal of this study is not to criticized the medical foundation model, but evaluate it in the wild to show the promise and perils. 

Fine-tuning has been an effective approach to leverage foundation models, however, due to the the extremely large size of the model, regular fine-tuning could be prohibitively costly for many research lab. Instead, another popular approach is to leverage the in-context learning ability of the foundation model through prompting. 
requires both substaintial downstream data as well as compute, a popular approach to work with foundation model is prompting \todo{Find reference}
\todo{Find more reference "goal of generalist model is to generalize to unseen task"}
\todo{Find reference: On serveral benchmarks, it is reported that the medical foundation model can be competitive or even surpass state-of-the-art (SOTA) specialist model. ~\cite{gruver2023large}}

UniDetector beats supervised
state-of-the-art models for large-vocabulary object detection
without being trained on training data and set new SOTA
for closed-vocabulary object detection.~\cite{wang2023detecting}

LLMs and vision-language models are excellent few-shot learners~\cite{brown2020language,awais2023foundational}, here we leverage the model's few shot in-context learning ability, equipped with prompting techniques. 


Flamingo shows excellent few-shot performance for
several vision-language tasks, even surpassing state-of-theart for fine-tuned models despite requiring significantly
fewer annotated examples~\cite{awais2023foundational}


A question has then arisen to the community “the foundation model approach” or “specialist model approach”. Prior work has shown both the promise as well as limitation of the foundation model approach toward medical problems~\cite{wu2023towards}. Therefore, it is important to evaluate such an approach on our specific task: diagnosing Aortic Stenosis. 

We experimented with Med-Flamingo~\cite{moor2023med} and RadFM~\cite{wu2023towards} using zero-shot, few-shot in-context prompting~\cite{brown2020language} and Chain-of-Thought (COT) prompting~\cite{wei2022chain}. However, despite substaintial effort in prompting, both Med-Flamingo and RadFM give chance performance. By a closer inspection, the model is not able to make sensible predictions. Example prompts used can be seen in App\todo{Prompts}. 

We then turn to an easier task: view classification task. Despite substaintial effort in prompting, no model can make view prediction accurately.

In our experiments, there are tasks that the model can achieve with high accuracy. e.g., recognizing the modailty of the image (ultrasound) \todo{~100\%?}; recognizing which part of the body is the image about\todo{~100\%?}

Our experiments show that the off-the-shelf foundation model do equip basic medical image knowledge, but still in its vary nascent stage, as noted by~\cite{wu2023towards}. 

These experiments is not to dismise the promise of the foundation model approach, but to test its performance in the wild. Further fine-tuning from these foundation model on specific down-stream task could be an effective alternative~\cite{wu2023towards}. Another promissing future direction could be a collaboration between human, specialist model and foundation model.


\begin{table}
\caption{Evaluating Off-the-shelf Medical Foundation Model}\label{tab1}
\begin{tabular}{l|c|c|c|c}
\hline
 &  AS Diagnosis & View Classification & Modality Recognition & Body Part Recognition \\
\hline
RadFM, zero-shot &  & & &\\
RadFM, 5-shot &  & & &\\
RadFM, COT &  & & &\\
Med-Flamingo, zero-shot &  & & &\\
Med-Flamingo, zero-shot &  & & &\\
Med-Flamingo, zero-shot &  & & &\\
\hline
\end{tabular}
\end{table}


==> SSL_workflow.tex <==
\begin{figure}[!t]
\centering
% \includesvg[width=1\textwidth]{figures/SAMIL_diagram_draft1.svg}
\includegraphics[width=0.8\textwidth]{figures/SMMIL_SSL.pdf}
\caption{\textbf{Overview of our Semi-Supervised Learning workflow.
}}%endcaption	
\label{fig:SSL_workflow}
\end{figure}

==> TMED2_AS_SeverityClassification.tex <==
\begin{table}[!h]
\parbox{.45\linewidth}{
\centering
    \caption{AS Severity Classification on TMED2 (Full-set). Showing balanced accuracy on the test set across three predefined train/test splits.
    }%endcaption
    \begin{tabular}{l|rrr| r }
	    & \multicolumn{4}{c}{Test Set Bal. Accuracy}\\
     Method & 1 & 2 & 3 & Avg (std)\\
    \hline
    ~\cite{holste2022automated} & 62.1 & 65.1 & 70.34 & 65.9 (3.4)
    \\
    % W. Avg. by View Rel.~\cite{wessler2023automated} $*$
    % & 74.46 & 72.61 & 76.24 & 74.43 (1.48) 
    % \\
    ~\cite{ilse2018attention}                 & 58.5 & 60.4 & 61.6 & 60.2 (1.3)\\
    ~\cite{ilse2018attention} Gated  & 57.8 & 62.6 & 59.8 & 60.0 (2.0)\\
    ~\cite{lee2019set} & 61.0 & 62.6 & 62.6 & 62.1 (0.8)\\
    ~\cite{li2021dual}  & 60.1 & 67.6 & 73.1 & 66.9 (5.3)\\
    ~\cite{huang2023detecting}            & 72.7 & 71.6 & 73.5 & 72.6 (0.8)\\
    % SAMIL~\cite{huang2023detecting}            & 75.41 & 73.78 & 79.42 & 76.20 (2.37)\\
    \hline
    SMMIL-I & \emph{81.7} & \emph{78.8} & \emph{85.6} & \emph{82.0} (2.8)\\
    SMMIL-V & \textbf{83.1} & \textbf{80.6} & \textbf{86.6} & \textbf{83.5} (2.5)\\
    \end{tabular}
    \label{tab:View Regularization ablation}
}%endparbox
\hfill 
\parbox{.45\linewidth}{
    \centering
    \caption{AS Severity Classification on TMED2 (clean-set). Showing balanced
    accuracy on the test set across three predefined train/test splits. ``--'' means not reported in the cited papers.
    }%endcaption
    \begin{tabular}{l|rrr| r }
	    & \multicolumn{4}{c}{Test Set Bal. Accuracy}\\
     Method & 1 & 2 & 3 & Avg (std)\\
    \hline
    ~\cite{wessler2023automated} 
    & 74.5 & 72.6 & 76.2 & 74.4 (1.5) \\
    ~\cite{vaseli2023protoasnet} 
    & 79.7 & --& -- & -- \\
    ~\cite{ahmadi2023transformer} 
    & 83.8 & -- & -- & -- \\
    \hline
    ~\cite{moor2023med} (zero) 
    & 50.0 & 50.0 & 50.0 & 50.0 (0) \\
    ~\cite{moor2023med} (COT) 
    & 50.0 & 50.0 & 50.0 & 50.0 (0) \\
    ~\cite{wu2023towards} (zero) 
    & 60.4 & 53.3 & 56.0 & 56.6 (2.9) \\
    \hline
    SMMIL-I & \emph{86.7} & \emph{82.8} & \textbf{87.7} & \emph{85.7} (2.1)\\
    SMMIL-V & \textbf{87.8} & \emph{82.1} & \textbf{89.6} & \textbf{86.5} (3.2)\\
    \end{tabular}
    \label{tab:Pretraining strategy ablation}
}%endparbox
\end{table}
